Non-linear response in extended systems: a real-time approach

In this thesis we present a new formalism to study linear and non-linear response in extended systems. Our approach is based on real-time solution of an effective Schr\"odinger equation. The coupling between electrons and external field is described by means of Modern Theory of Polarization. Correlation effects are derived from Green's function theory. We show that the inclusion of local-field effects and electron-hole interaction is crucial to predict and reproduce second and third harmonic generation in low dimensional structures, where strong bound excitons are present. Finally in the last part we introduce a real-time density functional approach suitable for infinite periodic crystals in which we work within the so-called length gauge and calculate the polarisation as a dynamical Berry's phase. This approach, in addition to the electron density considers also the macroscopic polarisation as a main variable to correctly treat periodic crystals in presence of electric fields within a density functional framework.

==> A <==
This is pdfTeX, Version 3.1415926-2.5-1.40.14 (TeX Live 2013/Debian)
 restricted \write18 enabled.
entering extended mode
(./hdr.tex
LaTeX2e <2011/06/27>
Babel <3.9h> and hyphenation patterns for 78 languages loaded.
(/usr/share/texlive/texmf-dist/tex/latex/base/book.cls
Document Class: book 2007/10/19 v1.4h Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/bk12.clo))
(/usr/share/texlive/texmf-dist/tex/latex/base/inputenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/utf8.def
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.dfu)
(/usr/share/texlive/texmf-dist/tex/latex/base/ot1enc.dfu)
(/usr/share/texlive/texmf-dist/tex/latex/base/omsenc.dfu)))
(/usr/share/texlive/texmf-dist/tex/latex/base/latexsym.sty)
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/biblatex2.sty
(/usr/share/texlive/texmf-dist/tex/latex/etoolbox/etoolbox.sty
(/usr/share/texlive/texmf-dist/tex/latex/etex-pkg/etex.sty))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvsetkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/etexcmds.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifluatex.sty))))
(/usr/share/texlive/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/share/texlive/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/bbx/alphabetic.bbx
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/bbx/standard.bbx))
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/cbx/alphabetic.cbx)
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/biblatex.cfg)))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/share/texlive/texmf-dist/tex/latex/was/gensymb.sty)
(/usr/share/texlive/texmf-dist/tex/latex/tools/enumerate.sty)
(/usr/share/texlive/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/lipsum/lipsum.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/color.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/pdftex-def/pdftex.def))
(/usr/share/texlive/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/graphics.cfg)))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/epsfig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/hyperref.cfg))

Package hyperref Message: Driver (autodetected): hpdftex.

(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/share/texlive/texmf-dist/tex/latex/biblatex/lbx/english.lbx) (./hdr.aux
(./introduction.aux) (./theory.aux) (./conclusions.aux)) (./hdr.bbl)

Package gensymb Warning: Not defining \perthousand.


Package gensymb Warning: Not defining \micro.

(/usr/share/texlive/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))
(./hdr.out) (./hdr.out) (./hdr.toc
(/usr/share/texlive/texmf-dist/tex/latex/base/ulasy.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)) [1{/var/lib/texmf/f
onts/map/pdftex/updmap/pdftex.map}] (./introduction.tex [2] [3] [4]
Chapter 1.
<immerse.png, id=117, 458.513pt x 290.686pt> <use immerse.png>
Underfull \hbox (badness 10000) in paragraph at lines 67--74
\OT1/cmr/m/n/12 field lines and cre-ate an in-ter-nal field,
[5 <./immerse.png>]

LaTeX Warning: Citation 'lee2014first' on page 6 undefined on input line 90.

<SHG_franken.png, id=133, 722.7pt x 216.05719pt> <use SHG_franken.png>

LaTeX Warning: Citation 'franken1961generation' on page 6 undefined on input li
ne 95.


LaTeX Warning: Citation 'franken1961generation' on page 6 undefined on input li
ne 95.

[6 <./SHG_franken.png>]

LaTeX Warning: Citation 'franken1961generation' on page 7 undefined on input li
ne 103.


LaTeX Warning: Citation 'maiman1960stimulated' on page 7 undefined on input lin
e 103.

<lasergreen.png, id=143, 561.89925pt x 407.121pt> <use lasergreen.png>

LaTeX Warning: Citation 'bloembergen1982nonlinear' on page 7 undefined on input
 line 114.


LaTeX Warning: Citation 'pantazis2010second' on page 7 undefined on input line 
125.


Overfull \hbox (106.95554pt too wide) in paragraph at lines 114--126
\OT1/cmr/m/n/12 of non-linear spectroscopy[[]

Underfull \hbox (badness 2521) in paragraph at lines 114--126
\OT1/cmr/m/n/12 ] made pro-gresses in leaps and

Underfull \hbox (badness 1527) in paragraph at lines 114--126
\OT1/cmr/m/n/12 con-fer-ences. In this de-vice the
[7 <./lasergreen.png>]

LaTeX Warning: Citation 'PhysRevLett.75.4337' on page 8 undefined on input line
 128.

<ferroelectric.png, id=152, 717.43031pt x 515.67656pt> <use ferroelectric.png>
Underfull \hbox (badness 10000) in paragraph at lines 128--136


LaTeX Warning: Citation 'yin2014edge' on page 8 undefined on input line 142.


Package wrapfig Warning: Collision between wrapping environments on input line 
143.

<mos2.png, id=155, 800.9925pt x 401.5pt> <use mos2.png>

LaTeX Warning: Citation 'yin2014edge' on page 8 undefined on input line 148.


LaTeX Warning: Citation 'yin2014edge' on page 8 undefined on input line 148.

[8 <./ferroelectric.png>]

Package wrapfig Warning: Stationary wrapfigure forced to float on input line 14
9.


LaTeX Warning: Citation 'doi:10.1021/nl401561r' on page 9 undefined on input li
ne 150.


LaTeX Warning: Citation 'eisenthal1996liquid' on page 9 undefined on input line
 151.


LaTeX Warning: Citation 'wang2005optical' on page 9 undefined on input line 152
.


LaTeX Warning: Citation 'cassabois2015hexagonal' on page 9 undefined on input l
ine 152.


Overfull \hbox (0.76555pt too wide) in paragraph at lines 149--156
\OT1/cmr/m/n/12 that are dark in lin-ear optics.[[]; []
[9]

LaTeX Warning: Citation 'encylaser' on page 10 undefined on input line 158.


Package wrapfig Warning: Collision between wrapping environments on input line 
159.

<selffocus.png, id=169, 278.641pt x 252.945pt> <use selffocus.png>
Underfull \hbox (badness 10000) in paragraph at lines 158--166


Package wrapfig Warning: Stationary wrapfigure forced to float on input line 16
6.


LaTeX Warning: Citation 'boyd' on page 10 undefined on input line 167.


LaTeX Warning: Citation 'bloembergen1982nonlinear' on page 10 undefined on inpu
t line 167.


Package wrapfig Warning: Stationary wrapfigure forced to float on input line 16
8.


LaTeX Warning: Citation 'bloembergen1964quantum' on page 10 undefined on input 
line 169.


LaTeX Warning: Citation 'PhysRev.126.413' on page 10 undefined on input line 16
9.


LaTeX Warning: Citation 'wiser1963dielectric' on page 10 undefined on input lin
e 169.


LaTeX Warning: Citation 'karplus1948note' on page 10 undefined on input line 16
9.


LaTeX Warning: Citation 'kubo1954general' on page 10 undefined on input line 16
9.


LaTeX Warning: Citation 'RevModPhys.33.249' on page 10 undefined on input line 
169.


LaTeX Warning: Citation 'PhysRev.102.104' on page 10 undefined on input line 16
9.


LaTeX Warning: Citation 'neumann' on page 10 undefined on input line 171.


Underfull \hbox (badness 1622) in paragraph at lines 169--173
\OT1/cmr/m/n/12 formalism.[[] ]

Underfull \hbox (badness 7851) in paragraph at lines 169--173
\OT1/cmr/m/n/12 This for-mal-ism was al-ready used in

Underfull \hbox (badness 5374) in paragraph at lines 169--173
\OT1/cmr/m/n/12 the past to de-rive lo-cal field ef-fects

Overfull \hbox (70.88336pt too wide) in paragraph at lines 169--173
\OT1/cmr/m/n/12 in lin-ear optics[[]; []

Underfull \hbox (badness 2744) in paragraph at lines 169--173
\OT1/cmr/m/n/12 ], to in-ves-ti-gate a non-linear phe-nom-

Overfull \hbox (92.01617pt too wide) in paragraph at lines 169--173
\OT1/cmr/m/n/12 ena like sat-u-ra-tion of mi-crowave resonances[[]

Underfull \hbox (badness 7704) in paragraph at lines 169--173
\OT1/cmr/m/n/12 ], and to de-scribe nu-clear mag-netic

Overfull \hbox (59.55579pt too wide) in paragraph at lines 169--173
\OT1/cmr/m/n/12 relaxation[[]; [];
[10 <./mos2.png> <./selffocus.png>]

LaTeX Warning: Citation 'tokman' on page 11 undefined on input line 182.


LaTeX Warning: Citation 'PhysRevB.56.1787' on page 11 undefined on input line 1
91.


LaTeX Warning: Citation 'PhysRevB.42.3567' on page 11 undefined on input line 1
91.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 11 undefined on input line
 191.


LaTeX Warning: Citation 'PhysRevB.50.5756' on page 11 undefined on input line 1
93.


LaTeX Warning: Citation 'andrade2007time' on page 11 undefined on input line 19
4.


LaTeX Warning: Citation 'takimoto:154114' on page 11 undefined on input line 19
6.


LaTeX Warning: Citation 'ding2013efficient' on page 11 undefined on input line 
196.


LaTeX Warning: Citation 'goncharov2013nonlinear' on page 11 undefined on input 
line 196.


LaTeX Warning: Citation 'nloptics2013' on page 11 undefined on input line 197.


Underfull \hbox (badness 4940) in paragraph at lines 188--198
\OT1/cmr/m/n/12 However in last years dif-fer-ent works ap-peared in the lit-er
-a-ture

Underfull \hbox (badness 1571) in paragraph at lines 188--198
\OT1/cmr/m/n/12 that use real-time prop-a-ga-tion to cal-cu-late non-linear re-
sponse both

Underfull \hbox (badness 5832) in paragraph at lines 188--198
\OT1/cmr/m/n/12 for molecular[[]; [] ] and pe-ri-odic
[11] [12]

LaTeX Warning: Citation 'PhysRevB.12.2325' on page 13 undefined on input line 2
01.


LaTeX Warning: Citation 'PhysRevB.36.9708' on page 13 undefined on input line 2
01.


LaTeX Warning: Citation 'PhysRevB.42.3567' on page 13 undefined on input line 2
02.


LaTeX Warning: Citation 'PhysRevB.61.5337' on page 13 undefined on input line 2
02.


LaTeX Warning: Citation 'PhysRevB.48.11705' on page 13 undefined on input line 
202.


LaTeX Warning: Citation 'PhysRevLett.63.1719' on page 13 undefined on input lin
e 203.


LaTeX Warning: Citation 'PhysRevB.56.1787' on page 13 undefined on input line 2
03.


LaTeX Warning: Citation 'strinati' on page 13 undefined on input line 204.


LaTeX Warning: Citation 'Chang2002' on page 13 undefined on input line 204.


LaTeX Warning: Citation 'Leitsmann2005' on page 13 undefined on input line 204.



LaTeX Warning: Citation 'PhysRevA.83.062122' on page 13 undefined on input line
 205.


LaTeX Warning: Citation 'PhysRevB.56.1787' on page 13 undefined on input line 2
05.


LaTeX Warning: Citation 'PhysRevLett.52.997' on page 13 undefined on input line
 206.


LaTeX Warning: Citation 'botti2007time' on page 13 undefined on input line 206.



LaTeX Warning: Citation 'botti2007time' on page 13 undefined on input line 206.



LaTeX Warning: Citation 'faber2014excited' on page 13 undefined on input line 2
06.


LaTeX Warning: Reference `chaptertddft' on page 13 undefined on input line 206.



LaTeX Warning: Citation 'takimoto:154114' on page 13 undefined on input line 20
7.


LaTeX Warning: Citation 'andrade2007time' on page 13 undefined on input line 20
7.

)
Overfull \hbox (11.79446pt too wide) in paragraph at lines 200--267
\OT1/cmr/m/n/12 by one or two or-der of magnitudes.[[]; []

Overfull \hbox (16.0585pt too wide) in paragraph at lines 200--267
\OT1/cmr/m/n/12 low-ing this idea Chang et al.[[] ] and Leits-man et al.[[]

Overfull \hbox (50.44243pt too wide) in paragraph at lines 200--267
\OT1/cmr/m/n/12 Sipe de-rived a sim-i-lar equa-tion for the third har-monic gen
eration.[[]

Overfull \hbox (103.242pt too wide) in paragraph at lines 200--267
\OT1/cmr/m/n/12 func-tion the-ory, is Time-Dependent Den-sity Func-tional The-o
ry (TDDFT)[[]
[13] [14] (./realtime.tex
Chapter 2.

LaTeX Warning: Citation 'kremp' on page 15 undefined on input line 4.


Overfull \hbox (2.71815pt too wide) in paragraph at lines 4--6
\OT1/cmr/m/n/12 In this sec-tion we present a sim-ple in-tro-duc-tion to the no
n-equilibrium Green's

LaTeX Warning: Reference `fullH' on page 15 undefined on input line 11.

[15]

LaTeX Warning: Citation 'neumann' on page 16 undefined on input line 32.


LaTeX Warning: Reference `densmat' on page 16 undefined on input line 37.


LaTeX Warning: Reference `densmat' on page 16 undefined on input line 37.


LaTeX Warning: Citation 'bonitz' on page 16 undefined on input line 37.


LaTeX Warning: Reference `densmat' on page 16 undefined on input line 39.

[16]

LaTeX Warning: Citation 'bonitz' on page 17 undefined on input line 43.


LaTeX Warning: Citation 'RevModPhys.74.895' on page 17 undefined on input line 
43.


Overfull \hbox (20.7365pt too wide) detected at line 52
[]\OML/cmm/m/it/12 G[]\OT1/cmr/m/n/12 (\OT1/cmr/bx/n/12 r[]\OML/cmm/m/it/12 ; t
[]:::\OT1/cmr/bx/n/12 r[]\OML/cmm/m/it/12 ; t[]; \OT1/cmr/bx/n/12 r[]\OML/cmm/m
/it/12 ; t[]:::\OT1/cmr/bx/n/12 r[]\OML/cmm/m/it/12 ; t[]\OT1/cmr/m/n/12 ) = []
[] \OMS/cmsy/m/n/12 h\OML/cmm/m/it/12  []\OT1/cmr/m/n/12 (\OT1/cmr/bx/n/12 r[]\
OML/cmm/m/it/12 ; t[]\OT1/cmr/m/n/12 )\OML/cmm/m/it/12 ::: []\OT1/cmr/m/n/12 (\
OT1/cmr/bx/n/12 r[]\OML/cmm/m/it/12 ; t[]\OT1/cmr/m/n/12 )\OML/cmm/m/it/12  \OT
1/cmr/m/n/12 (\OT1/cmr/bx/n/12 r[]\OML/cmm/m/it/12 ; t[]\OT1/cmr/m/n/12 )\OML/c
mm/m/it/12 ::: \OT1/cmr/m/n/12 (\OT1/cmr/bx/n/12 r[]\OML/cmm/m/it/12 ; t[]\OT1/
cmr/m/n/12 )\OMS/cmsy/m/n/12 i\OML/cmm/m/it/12 :

LaTeX Warning: Citation 'kremp' on page 17 undefined on input line 54.

[17]

LaTeX Warning: Reference `kbeq' on page 18 undefined on input line 65.


LaTeX Warning: Citation 'kremp' on page 18 undefined on input line 65.


LaTeX Warning: Citation 'schafer' on page 18 undefined on input line 65.


LaTeX Warning: Citation 'kadanoff' on page 18 undefined on input line 65.


LaTeX Warning: Citation 'haug2008quantum' on page 18 undefined on input line 65
.


LaTeX Warning: Reference `kbeq' on page 18 undefined on input line 66.


LaTeX Warning: Citation 'aryasetiawan1998gw' on page 18 undefined on input line
 68.


LaTeX Warning: Citation 'hedin1999correlation' on page 18 undefined on input li
ne 68.


LaTeX Warning: Citation 'PhysRevB.25.2867' on page 18 undefined on input line 6
8.


LaTeX Warning: Citation 'aryasetiawan1998gw' on page 18 undefined on input line
 68.


LaTeX Warning: Citation 'Aulbur19991' on page 18 undefined on input line 68.


LaTeX Warning: Citation 'faber2011first' on page 18 undefined on input line 68.



LaTeX Warning: Citation 'faber2015exploring' on page 18 undefined on input line
 68.


LaTeX Warning: Citation 'PhysRevB.69.205204' on page 18 undefined on input line
 69.


Overfull \hbox (25.87888pt too wide) in paragraph at lines 64--70
\OT1/cmr/m/n/12 cor-rec-tions have shown a clear im-prove-ment for band gaps[[]
;
[18]

LaTeX Warning: Citation 'PhysRevB.62.7998' on page 19 undefined on input line 7
5.


LaTeX Warning: Citation 'PSSB:PSSB200642067' on page 19 undefined on input line
 75.


LaTeX Warning: Citation 'sun:234107' on page 19 undefined on input line 75.


LaTeX Warning: Citation 'strinati' on page 19 undefined on input line 76.


LaTeX Warning: Citation 'takimoto:154114' on page 19 undefined on input line 78
.


LaTeX Warning: Citation 'PSSB:PSSB200642067' on page 19 undefined on input line
 79.


LaTeX Warning: Reference `chaptertddft' on page 19 undefined on input line 80.


LaTeX Warning: Citation 'Aulbur19991' on page 19 undefined on input line 85.


LaTeX Warning: Citation 'PhysRevLett.45.290' on page 19 undefined on input line
 86.


LaTeX Warning: Citation 'Aulbur19991' on page 19 undefined on input line 87.


LaTeX Warning: Citation 'faber2013many' on page 19 undefined on input line 87.


LaTeX Warning: Citation 'strinati' on page 19 undefined on input line 89.


Overfull \hbox (35.21977pt too wide) in paragraph at lines 74--91
\OT1/cmr/m/n/12 many-body per-tur-ba-tion the-ory (MBPT) within the lin-ear re-
sponse regime [[]

Overfull \hbox (25.68558pt too wide) in paragraph at lines 74--91
\OT1/cmr/m/n/12 to in-ves-ti-gate non-lin-ear ef-fects like sec-ond har-monic g
eneration[[]

Overfull \hbox (117.03659pt too wide) in paragraph at lines 74--91
\OT1/cmr/m/n/12 approximation[[] ]. Since its first ap-pli-ca-tion to semicondu
ctors[[]

Overfull \hbox (24.01733pt too wide) in paragraph at lines 74--91
\OT1/cmr/m/n/12 er-gies and life-times for a wide range of materials[[]; []

LaTeX Warning: Citation 'Onida' on page 19 undefined on input line 93.


LaTeX Warning: Citation 'Chang2002' on page 19 undefined on input line 95.


LaTeX Warning: Citation 'Leitsmann2005' on page 19 undefined on input line 95.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 19 undefined on input line
 95.


LaTeX Warning: Citation 'kadanoffbaym' on page 19 undefined on input line 96.


LaTeX Warning: Citation 'kadanoffbaym' on page 19 undefined on input line 97.

[19]

LaTeX Warning: Citation 'PhysRevB.37.941' on page 20 undefined on input line 10
5.


LaTeX Warning: Citation 'PhysRevB.58.2064' on page 20 undefined on input line 1
06.


LaTeX Warning: Citation 'PhysRevB.38.9759' on page 20 undefined on input line 1
07.


LaTeX Warning: Citation 'PhysRevLett.86.2451' on page 20 undefined on input lin
e 107.


LaTeX Warning: Citation 'Kohler1999123' on page 20 undefined on input line 108.



LaTeX Warning: Citation 'PhysRevLett.103.176404' on page 20 undefined on input 
line 108.


LaTeX Warning: Citation 'PhysRevLett.84.1768' on page 20 undefined on input lin
e 108.


LaTeX Warning: Citation 'PhysRevLett.98.153004' on page 20 undefined on input l
ine 108.


LaTeX Warning: Reference `tdbse_section' on page 20 undefined on input line 111
.


LaTeX Warning: Reference `linear_response' on page 20 undefined on input line 1
12.


LaTeX Warning: Reference `teospectro' on page 20 undefined on input line 114.


Overfull \hbox (88.63304pt too wide) in paragraph at lines 105--117
\OT1/cmr/m/n/12 nam-ics in real-time. [[]; []; [];
[20]
Overfull \hbox (5.59972pt too wide) in paragraph at lines 118--118
[]\OT1/cmr/bx/n/17.28 The time-dependent Bethe-Salpeter equa-

LaTeX Warning: Reference `ss:solution' on page 21 undefined on input line 128.


LaTeX Warning: Reference `ss:KBEs' on page 21 undefined on input line 133.


LaTeX Warning: Citation 'kremp' on page 21 undefined on input line 133.


LaTeX Warning: Reference `ss:KS-CHSX' on page 21 undefined on input line 134.


LaTeX Warning: Reference `linear_response' on page 21 undefined on input line 1
39.


LaTeX Warning: Citation 'PhysRevB.67.085307' on page 21 undefined on input line
 142.


LaTeX Warning: Citation 'kadanoffbaym' on page 21 undefined on input line 148.


LaTeX Warning: Citation 'kremp' on page 21 undefined on input line 148.


LaTeX Warning: Citation 'schafer' on page 21 undefined on input line 148.


Overfull \hbox (9.30649pt too wide) detected at line 157
[] [][] \OMS/cmsy/m/n/12 ^^Q \OML/cmm/m/it/12 G[]\OT1/cmr/m/n/12 (\OML/cmm/m/it
/12 t[]; t[]\OT1/cmr/m/n/12 ) = [] \OML/cmm/m/it/12 '[]\OT1/cmr/m/n/12 (\OT1/cm
r/bx/n/12 r[]\OT1/cmr/m/n/12 )\OML/cmm/m/it/12 G [] '[]\OT1/cmr/m/n/12 (\OT1/cm
r/bx/n/12 r[]\OT1/cmr/m/n/12 )d[]\OML/cmm/m/it/12 r[]\OT1/cmr/m/n/12 d[]\OML/cm
m/m/it/12 r[]:

LaTeX Warning: Reference `GFdefinition' on page 21 undefined on input line 160.



LaTeX Warning: Citation 'kremp' on page 21 undefined on input line 172.

[21]

LaTeX Warning: Reference `eqden' on page 22 undefined on input line 184.


LaTeX Warning: Reference `eqmotGone' on page 22 undefined on input line 184.


LaTeX Warning: Citation 'Kohler1999123' on page 22 undefined on input line 187.



LaTeX Warning: Citation 'PhysRevLett.103.176404' on page 22 undefined on input 
line 187.


LaTeX Warning: Citation 'PhysRevLett.84.1768' on page 22 undefined on input lin
e 187.


LaTeX Warning: Citation 'PhysRevLett.98.153004' on page 22 undefined on input l
ine 187.


LaTeX Warning: Citation 'Kohler1999123' on page 22 undefined on input line 188.



LaTeX Warning: Citation 'PhysRevLett.103.176404' on page 22 undefined on input 
line 188.


LaTeX Warning: Citation 'PhysRevLett.84.1768' on page 22 undefined on input lin
e 188.


LaTeX Warning: Citation 'PhysRevLett.98.153004' on page 22 undefined on input l
ine 188.


Overfull \hbox (3.2252pt too wide) in paragraph at lines 186--190
\OT1/cmr/m/n/12 systems[[]; [] ], in the ho-mo-ge-neous

Overfull \hbox (16.04022pt too wide) in paragraph at lines 186--190
\OT1/cmr/m/n/12 elec-tron gas[[] ], and in atoms[[]

Overfull \hbox (31.13696pt too wide) in paragraph at lines 186--190
[]\OT1/cmr/m/n/12 ; []; []
[22]

LaTeX Warning: Reference `hamiltonian' on page 23 undefined on input line 196.


LaTeX Warning: Citation 'PhysRev.140.A1133' on page 23 undefined on input line 
196.


LaTeX Warning: Reference `eqmotGone' on page 23 undefined on input line 216.


LaTeX Warning: Citation 'PhysRevB.38.7530' on page 23 undefined on input line 2
24.


LaTeX Warning: Reference `eq:appcsx' on page 23 undefined on input line 224.

[23]

LaTeX Warning: Citation 'kremp' on page 24 undefined on input line 233.


LaTeX Warning: Citation 'PhysRevB.38.7530' on page 24 undefined on input line 2
34.


LaTeX Warning: Citation 'PhysRevB.69.205204' on page 24 undefined on input line
 234.


Overfull \hbox (9.91022pt too wide) in paragraph at lines 230--235
\OT1/cmr/m/n/12 the $\OML/cmm/m/it/12 GW$ \OT1/cmr/m/n/12 self-energy (see Ch.4
 of Ref. [[] ] and Refs. [[];

LaTeX Warning: Reference `eq:appcsx' on page 24 undefined on input line 236.


LaTeX Warning: Reference `eq:appret' on page 24 undefined on input line 236.


LaTeX Warning: Reference `eqmotGone' on page 24 undefined on input line 236.


LaTeX Warning: Reference `eqmotGone' on page 24 undefined on input line 237.


LaTeX Warning: Reference `eqmotGcohsex' on page 24 undefined on input line 253.



LaTeX Warning: Reference `eqmotGcohsex' on page 24 undefined on input line 259.



LaTeX Warning: Citation 'PhysRevLett.45.290' on page 24 undefined on input line
 262.


LaTeX Warning: Citation 'PhysRevLett.91.176402' on page 24 undefined on input l
ine 262.


LaTeX Warning: Citation 'bsedynamic' on page 24 undefined on input line 272.


LaTeX Warning: Citation 'PhysRevB.77.115118' on page 24 undefined on input line
 272.


LaTeX Warning: Citation 'PhysRevLett.91.176402' on page 24 undefined on input l
ine 273.


Overfull \hbox (42.95251pt too wide) in paragraph at lines 252--274
\OT1/cmr/m/n/12 tion to an op-po-site en-hance-ment of the op-ti-cal prop-er-ti
es. [[]
[24]

LaTeX Warning: Reference `eqmotGcohsex' on page 25 undefined on input line 275.



LaTeX Warning: Citation 'Onida' on page 25 undefined on input line 282.


LaTeX Warning: Reference `coh_anx_sex' on page 25 undefined on input line 283.


LaTeX Warning: Citation 'Onida' on page 25 undefined on input line 290.


LaTeX Warning: Reference `tdbse' on page 25 undefined on input line 296.


LaTeX Warning: Reference `tdbse' on page 25 undefined on input line 302.


LaTeX Warning: Reference `tdbse' on page 25 undefined on input line 304.


LaTeX Warning: Citation 'Onida' on page 25 undefined on input line 307.


LaTeX Warning: Citation 'Aulbur19991' on page 25 undefined on input line 307.


LaTeX Warning: Reference `tdbse' on page 25 undefined on input line 308.

[25]

LaTeX Warning: Reference `mbhamiltonian' on page 26 undefined on input line 314
.


LaTeX Warning: Reference `ss:solution' on page 26 undefined on input line 315.


LaTeX Warning: Reference `tdbse' on page 26 undefined on input line 335.


LaTeX Warning: Reference `tdbse' on page 26 undefined on input line 342.


LaTeX Warning: Citation 'strinati' on page 26 undefined on input line 342.


LaTeX Warning: Citation 'Aulbur19991' on page 26 undefined on input line 342.


LaTeX Warning: Citation 'bsedynamic' on page 26 undefined on input line 343.


LaTeX Warning: Reference `hamiltonian' on page 26 undefined on input line 351.


LaTeX Warning: Citation 'PhysRevLett.84.1768' on page 26 undefined on input lin
e 376.


LaTeX Warning: Reference `basisChi' on page 26 undefined on input line 377.


LaTeX Warning: Reference `eqden' on page 26 undefined on input line 377.


LaTeX Warning: Reference `eq:phychi' on page 26 undefined on input line 377.

[26]

LaTeX Warning: Reference `tdbse' on page 27 undefined on input line 385.


LaTeX Warning: Reference `eq:sciss' on page 27 undefined on input line 392.


LaTeX Warning: Reference `gtilde' on page 27 undefined on input line 392.


LaTeX Warning: Reference `DDcorFun_n' on page 27 undefined on input line 392.


LaTeX Warning: Reference `diag_contr' on page 27 undefined on input line 401.


LaTeX Warning: Reference `dtGtt' on page 27 undefined on input line 401.


LaTeX Warning: Reference `DDcorFun_n' on page 27 undefined on input line 401.


Overfull \hbox (3.12292pt too wide) detected at line 405
 []$[]  \OML/cmm/m/it/12 ^^NV[] [] \OT1/cmr/m/n/12 = [] [] []  \OML/cmm/m/it/12
 dt[] dt[][] \OMS/cmsy/m/n/12 ^^B \OML/cmm/m/it/12 ^^_[]\OT1/cmr/m/n/12 (\OML/c
mm/m/it/12 t[]; t[]\OT1/cmr/m/n/12 )\OML/cmm/m/it/12 ^^NU[] [] ;$ [][][]  

LaTeX Warning: Reference `V_exp' on page 27 undefined on input line 407.

[27]

LaTeX Warning: Reference `eq:chimat' on page 28 undefined on input line 412.


LaTeX Warning: Reference `eq:hrtrG' on page 28 undefined on input line 413.


LaTeX Warning: Reference `eq:hrtrG' on page 28 undefined on input line 415.


LaTeX Warning: Reference `V_exp' on page 28 undefined on input line 415.


Package pdftex.def Warning: Option `bbllx' is not supported, use
(pdftex.def)                option `viewport' instead on input line 424.


Package pdftex.def Warning: Option `bblly' is not supported, use
(pdftex.def)                option `viewport' instead on input line 424.


Package pdftex.def Warning: Option `bburx' is not supported, use
(pdftex.def)                option `viewport' instead on input line 424.


Package pdftex.def Warning: Option `bbury' is not supported, use
(pdftex.def)                option `viewport' instead on input line 424.

<tdh-eps-converted-to.pdf, id=306, 626.34pt x 251.94125pt>
<use tdh-eps-converted-to.pdf>

Package pdftex.def Warning: Option `bbllx' is not supported, use
(pdftex.def)                option `viewport' instead on input line 425.


Package pdftex.def Warning: Option `bblly' is not supported, use
(pdftex.def)                option `viewport' instead on input line 425.


Package pdftex.def Warning: Option `bburx' is not supported, use
(pdftex.def)                option `viewport' instead on input line 425.


Package pdftex.def Warning: Option `bbury' is not supported, use
(pdftex.def)                option `viewport' instead on input line 425.

<bse-eps-converted-to.pdf, id=308, 626.34pt x 251.94125pt>
<use bse-eps-converted-to.pdf>
Overfull \hbox (36.79134pt too wide) in paragraph at lines 424--433
 [][] 

Overfull \hbox (36.79134pt too wide) in paragraph at lines 424--433
 [] 

LaTeX Warning: Citation 'attaccalite' on page 28 undefined on input line 433.


LaTeX Warning: Citation 'attaccalite' on page 28 undefined on input line 433.


LaTeX Warning: Reference `fastcohsex' on page 28 undefined on input line 437.


LaTeX Warning: Citation 'strinati' on page 28 undefined on input line 443.


Overfull \hbox (7.27643pt too wide) in paragraph at lines 442--444
\OT1/cmr/m/n/12 where we ne-glected the part con-tain-ing the func-tional deriv
a-tive of the screened

LaTeX Warning: Reference `diag_contr' on page 28 undefined on input line 445.


LaTeX Warning: Reference `H_contr' on page 28 undefined on input line 445.


LaTeX Warning: Reference `xc_contr' on page 28 undefined on input line 445.


LaTeX Warning: Reference `dtGtt' on page 28 undefined on input line 445.


Overfull \hbox (1.44774pt too wide) in paragraph at lines 466--466
[]\OT1/cmr/bx/n/17.28 Optical prop-er-ties from a time-dependent

LaTeX Warning: Reference `mbhamiltonian' on page 28 undefined on input line 469
.

[28]

LaTeX Warning: Citation 'blount' on page 29 undefined on input line 472.


LaTeX Warning: Citation 'souza_prb' on page 29 undefined on input line 473.


LaTeX Warning: Citation 'nloptics2013' on page 29 undefined on input line 473.


LaTeX Warning: Reference `mbhamiltonian' on page 29 undefined on input line 473
.


LaTeX Warning: Citation 'PhysRevLett.87.036401' on page 29 undefined on input l
ine 480.


LaTeX Warning: Citation 'PhysRevLett.84.1768' on page 29 undefined on input lin
e 481.


LaTeX Warning: Citation 'PhysRevLett.96.126104' on page 29 undefined on input l
ine 487.


LaTeX Warning: Citation 'PhysRevLett.100.189701' on page 29 undefined on input 
line 487.


LaTeX Warning: Citation 'attaccalite' on page 29 undefined on input line 487.


LaTeX Warning: Reference `tdbse_shf' on page 29 undefined on input line 488.


LaTeX Warning: Reference `linear_response' on page 29 undefined on input line 4
93.


Overfull \hbox (2.94405pt too wide) in paragraph at lines 476--494
[]\OT1/cmr/m/n/12 ; [] ]. In this ex-am-ple we used Eq. [],
[29]

LaTeX Warning: Reference `hbn' on page 30 undefined on input line 495.


LaTeX Warning: Reference `linear_response' on page 30 undefined on input line 5
04.


LaTeX Warning: Citation 'attaccalite' on page 30 undefined on input line 506.


LaTeX Warning: Reference `hbn' on page 30 undefined on input line 506.


LaTeX Warning: Reference `hbn' on page 30 undefined on input line 506.


LaTeX Warning: Reference `hbn' on page 30 undefined on input line 508.


LaTeX Warning: Reference `hbn' on page 30 undefined on input line 508.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 512.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `subscript' on input line 512.


Package hyperref Warning: Token not allowed in a PDF string (PDFDocEncoding):
(hyperref)                removing `math shift' on input line 512.


LaTeX Warning: Citation 'attaccalite2015strong' on page 30 undefined on input l
ine 513.


LaTeX Warning: Citation 'gruning2014erratum' on page 30 undefined on input line
 513.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 30 undefined on input line
 513.


LaTeX Warning: Citation 'doi:10.1021/nn403159y' on page 30 undefined on input l
ine 514.


LaTeX Warning: Citation 'PhysRevB.87.201401' on page 30 undefined on input line
 514.


LaTeX Warning: Citation 'doi:10.1021/nn403159y' on page 30 undefined on input l
ine 515.


Overfull \hbox (63.48734pt too wide) in paragraph at lines 513--516
\OT1/cmr/m/n/12 tion(SHG) in two di-men-sional crystals.[[]; [];

Overfull \hbox (46.75937pt too wide) in paragraph at lines 513--516
\OT1/cmr/m/n/12 lute terms is in-her-ently weak, though rel-a-tively very stron
g.[[]
[30] <exciton.pdf, id=335, 535.57745pt x 375.73029pt> <use exciton.pdf>
Underfull \hbox (badness 1365) in paragraph at lines 522--522
\OT1/cmr/m/n/10 (dark red) into the fun-da-men-tal

LaTeX Warning: Citation 'doi:10.1021/nl401561r' on page 31 undefined on input l
ine 526.


LaTeX Warning: Citation 'kumar2013second' on page 31 undefined on input line 52
6.


LaTeX Warning: Citation 'PhysRevLett.96.126104' on page 31 undefined on input l
ine 531.


LaTeX Warning: Citation 'PhysRevLett.100.189701' on page 31 undefined on input 
line 531.


LaTeX Warning: Citation 'PhysRevLett.105.136805' on page 31 undefined on input 
line 531.


LaTeX Warning: Citation 'molina2013effect' on page 31 undefined on input line 5
31.


Underfull \hbox (badness 4084) in paragraph at lines 531--532
\OT1/cmr/m/n/12 two ma-te-ri-als share an hexag-o-nal 2D

Underfull \hbox (badness 1502) in paragraph at lines 531--532
\OT1/cmr/m/n/12 struc-ture but their elec-tronic and op-ti-

Underfull \hbox (badness 1052) in paragraph at lines 531--532
\OT1/cmr/m/n/12 cal prop-er-ties are quite dif-fer-ent. The

Overfull \hbox (113.94617pt too wide) in paragraph at lines 531--532
\OT1/cmr/m/n/12 excitons.[[]; []

LaTeX Warning: Citation 'molina2013effect' on page 31 undefined on input line 5
33.


LaTeX Warning: Citation 'PhysRevLett.100.189701' on page 31 undefined on input 
line 533.


LaTeX Warning: Citation 'scholes2006excitons' on page 31 undefined on input lin
e 533.


LaTeX Warning: Citation 'guo2005second' on page 31 undefined on input line 537.



LaTeX Warning: Citation 'margulis2013optical' on page 31 undefined on input lin
e 537.


LaTeX Warning: Reference `schemeshg' on page 31 undefined on input line 537.


LaTeX Warning: Citation 'scholes2006excitons' on page 31 undefined on input lin
e 537.


Overfull \hbox (47.67307pt too wide) in paragraph at lines 537--544
\OT1/cmr/m/n/12 ploy the in-de-pen-dent par-ti-cle approximation[[]; []

Overfull \hbox (83.02016pt too wide) in paragraph at lines 537--544
\OT1/cmr/m/n/12 ] (IPA) which are in-ad-e-quate for low di-men-sional sys-tems 
(see Fig. []).[[]
[31 <./exciton.pdf>]

LaTeX Warning: Reference `mbhamiltonian' on page 32 undefined on input line 561
.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 32 undefined on input line
 561.


LaTeX Warning: Citation 'PhysRevLett.96.126104' on page 32 undefined on input l
ine 565.


LaTeX Warning: Citation 'PhysRevLett.100.189701' on page 32 undefined on input 
line 565.

<eps_and_X2.pdf, id=369, 542.025pt x 1084.05pt> <use eps_and_X2.pdf>

LaTeX Warning: Reference `mbhamiltonian' on page 32 undefined on input line 571
.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 32 undefined on input line
 571.


LaTeX Warning: Reference `mbhamiltonian' on page 32 undefined on input line 571
.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 32 undefined on input line
 571.


Overfull \hbox (108.22961pt too wide) in paragraph at lines 565--572
\OT1/cmr/m/n/12 ex-ci-tons and they are nearly in-de-pen-dent from the lay-ers 
arrangement.[[];

Underfull \vbox (badness 10000) has occurred while \output is active [32]
<IPX2.pdf, id=376, 542.025pt x 361.35pt> <use IPX2.pdf>

LaTeX Warning: Citation 'guo2005second' on page 33 undefined on input line 578.



LaTeX Warning: Citation 'PhysRevB.89.081102' on page 33 undefined on input line
 578.


LaTeX Warning: Citation 'guo2005second' on page 33 undefined on input line 578.



LaTeX Warning: Citation 'PhysRevB.89.081102' on page 33 undefined on input line
 578.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: Reference `absX2bn' on page 33 undefined on input line 580.

[33 <./eps_and_X2.pdf>]

LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 582.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 582.


LaTeX Warning: Citation 'guo2005second' on page 34 undefined on input line 587.



LaTeX Warning: Reference `X2bn' on page 34 undefined on input line 587.


LaTeX Warning: Citation 'guo2005second' on page 34 undefined on input line 587.



LaTeX Warning: Reference `mbhamiltonian' on page 34 undefined on input line 587
.

<absX2MoS2.pdf, id=463, 722.7pt x 722.7pt> <use absX2MoS2.pdf>

LaTeX Warning: Reference `mbhamiltonian' on page 34 undefined on input line 593
.


LaTeX Warning: Citation 'PhysRevB.87.201401' on page 34 undefined on input line
 593.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 34 undefined on input line
 593.


LaTeX Warning: Reference `mbhamiltonian' on page 34 undefined on input line 593
.


LaTeX Warning: Citation 'PhysRevB.87.201401' on page 34 undefined on input line
 593.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 34 undefined on input line
 593.


LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 597.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 597.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 597.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 597.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 34 undefined on input line
 597.


LaTeX Warning: Citation 'hughes1996calculation' on page 34 undefined on input l
ine 597.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 598.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 600.


LaTeX Warning: Reference `mbhamiltonian' on page 34 undefined on input line 600
.


LaTeX Warning: Citation 'strinati' on page 34 undefined on input line 600.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 600.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 600.


LaTeX Warning: Reference `absX2bn' on page 34 undefined on input line 600.


Underfull \vbox (badness 4621) has occurred while \output is active [34]

LaTeX Warning: Reference `mbhamiltonian' on page 35 undefined on input line 620
.


LaTeX Warning: Citation 'guo2005second' on page 35 undefined on input line 620.



LaTeX Warning: Reference `mbhamiltonian' on page 35 undefined on input line 620
.


LaTeX Warning: Citation 'guo2005second' on page 35 undefined on input line 620.



LaTeX Warning: Reference `tab1' on page 35 undefined on input line 624.


LaTeX Warning: Citation 'guo2005second' on page 35 undefined on input line 625.



LaTeX Warning: Citation 'PhysRevB.82.235201' on page 35 undefined on input line
 627.


LaTeX Warning: Citation 'LRC' on page 35 undefined on input line 627.


LaTeX Warning: Reference `absX2bn' on page 35 undefined on input line 627.


LaTeX Warning: Reference `absX2bn' on page 35 undefined on input line 627.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 35 undefined on input line
 627.


LaTeX Warning: Citation 'PhysRevLett.105.136805' on page 35 undefined on input 
line 630.


LaTeX Warning: Reference `fg:SHMoS2' on page 35 undefined on input line 631.


LaTeX Warning: Reference `mbhamiltonian' on page 35 undefined on input line 631
.


LaTeX Warning: Reference `fg:SHMoS2' on page 35 undefined on input line 631.


LaTeX Warning: Reference `mbhamiltonian' on page 35 undefined on input line 631
.


LaTeX Warning: Citation 'molina2013effect' on page 35 undefined on input line 6
32.


LaTeX Warning: Citation 'PhysRevB.87.201401' on page 35 undefined on input line
 632.


LaTeX Warning: Reference `fg:SHMoS2' on page 35 undefined on input line 633.


LaTeX Warning: Reference `fg:SHMoS2' on page 35 undefined on input line 636.


LaTeX Warning: Citation 'PhysRevLett.105.136805' on page 35 undefined on input 
line 636.


LaTeX Warning: Citation 'molina2013effect' on page 35 undefined on input line 6
36.


LaTeX Warning: Citation 'PhysRevB.87.201401' on page 35 undefined on input line
 636.


LaTeX Warning: Reference `fg:SHMoS2' on page 35 undefined on input line 636.


LaTeX Warning: Reference `absX2bn' on page 35 undefined on input line 637.


LaTeX Warning: Reference `fg:SHMoS2' on page 35 undefined on input line 637.

[35] [36]

LaTeX Warning: Citation 'bsedynamic' on page 37 undefined on input line 648.


LaTeX Warning: Citation 'giustino2016electron' on page 37 undefined on input li
ne 649.


LaTeX Warning: Citation 'gao2012artificially' on page 37 undefined on input lin
e 655.


LaTeX Warning: Citation 'gao2012artificially' on page 37 undefined on input lin
e 655.


LaTeX Warning: Citation 'nloptics2013' on page 37 undefined on input line 656.


LaTeX Warning: Citation 'attaccalite' on page 37 undefined on input line 656.


LaTeX Warning: Citation 'attaccalite2015strong' on page 37 undefined on input l
ine 657.


LaTeX Warning: Citation 'attaccalite1d' on page 37 undefined on input line 657.


)
Overfull \hbox (105.8199pt too wide) in paragraph at lines 639--269
\OT1/cmr/m/n/12 The in-ter-ested reader can find other ap-pli-ca-tions of the T
D-BSE in Refs. [[];
[37] [38] [39 <./tdh-eps-converted-to.pdf> <./bse-eps-converted-to.pdf>]
[40 <./IPX2.pdf>] [41 <./absX2MoS2.pdf>] (./tddft.tex [42]
Chapter 3.

LaTeX Warning: Citation 'PhysRev.140.A1133' on page 43 undefined on input line 
4.


LaTeX Warning: Citation 'PhysRev.136.B864' on page 43 undefined on input line 4
.


LaTeX Warning: Citation 'doi:10.1021/jp960669l' on page 43 undefined on input l
ine 4.


LaTeX Warning: Citation 'RevModPhys.87.897' on page 43 undefined on input line 
4.


LaTeX Warning: Citation 'PhysRevLett.52.997' on page 43 undefined on input line
 4.


LaTeX Warning: Citation 'Onida' on page 43 undefined on input line 4.


LaTeX Warning: Citation 'faber2014excited' on page 43 undefined on input line 4
.


LaTeX Warning: Citation 'valiev2010nwchem' on page 43 undefined on input line 4
.


LaTeX Warning: Citation 'PSSB:PSSB200642067' on page 43 undefined on input line
 4.


LaTeX Warning: Citation 'strinati' on page 43 undefined on input line 6.


LaTeX Warning: Citation 'Aulbur19991' on page 43 undefined on input line 6.


LaTeX Warning: Citation 'blase2011charge' on page 43 undefined on input line 6.



LaTeX Warning: Citation 'faber2012electron' on page 43 undefined on input line 
6.


LaTeX Warning: Citation 'maitra2003current' on page 43 undefined on input line 
8.


LaTeX Warning: Citation 'maitra2003current' on page 43 undefined on input line 
12.


LaTeX Warning: Citation 'PhysRevA.38.1149' on page 43 undefined on input line 1
3.


Overfull \hbox (11.79178pt too wide) in paragraph at lines 4--16
\OT1/cmr/m/n/12 Density func-tional the-ory (DFT)[[]; []

Overfull \hbox (3.58882pt too wide) in paragraph at lines 4--16
\OT1/cmr/m/n/12 and fi-nite systems[[]; [] ]. Time-

Overfull \hbox (16.8566pt too wide) in paragraph at lines 4--16
\OT1/cmr/m/n/12 have been en-coded in stan-dard quan-tum chem-i-cal packages[[]


Overfull \hbox (41.73218pt too wide) in paragraph at lines 4--16
\OT1/cmr/m/n/12 extended[[] ] and fi-nite systems[[]; []
[43] [44]

LaTeX Warning: Citation 'maitra2003current' on page 45 undefined on input line 
19.


LaTeX Warning: Citation 'PhysRevA.38.1149' on page 45 undefined on input line 1
9.


LaTeX Warning: Citation 'PhysRevLett.88.066404' on page 45 undefined on input l
ine 21.


LaTeX Warning: Citation 'PhysRevB.9.1998' on page 45 undefined on input line 21
.


LaTeX Warning: Citation 'Gonze1995' on page 45 undefined on input line 22.


Overfull \hbox (3.9473pt too wide) in paragraph at lines 19--23
\OT1/cmr/m/n/12 rents and po-ten-tials (scalar and vec-tor) can be es-tab-lishe
d and time-dependent
[45]

LaTeX Warning: Citation 'takimoto:154114' on page 46 undefined on input line 25
.


LaTeX Warning: Citation 'lee2014first' on page 46 undefined on input line 25.


LaTeX Warning: Citation 'otobe2015femtosecond' on page 46 undefined on input li
ne 25.


LaTeX Warning: Citation 'maitra2003current' on page 46 undefined on input line 
26.


LaTeX Warning: Citation 'PhysRevLett.115.137402' on page 46 undefined on input 
line 26.


LaTeX Warning: Citation 'LRC' on page 46 undefined on input line 26.


LaTeX Warning: Citation 'jgm' on page 46 undefined on input line 26.


LaTeX Warning: Citation 'Gonze1995' on page 46 undefined on input line 65.


LaTeX Warning: Citation 'Resta1996' on page 46 undefined on input line 65.


LaTeX Warning: Citation 'Vanderbilt1997' on page 46 undefined on input line 65.



LaTeX Warning: Citation 'Martin1997' on page 46 undefined on input line 65.


LaTeX Warning: Citation 'Martin1997' on page 46 undefined on input line 65.

[46]

LaTeX Warning: Citation 'Martin1997' on page 47 undefined on input line 72.


LaTeX Warning: Citation 'Martin1997' on page 47 undefined on input line 78.


LaTeX Warning: Citation 'Umari2005' on page 47 undefined on input line 78.


LaTeX Warning: Citation 'Martin1997' on page 47 undefined on input line 80.


LaTeX Warning: Reference `eq:dpftks' on page 47 undefined on input line 87.


LaTeX Warning: Reference `eq:dpftks' on page 47 undefined on input line 96.


LaTeX Warning: Reference `eq:dpften' on page 47 undefined on input line 96.

[47]

LaTeX Warning: Citation 'PhysRevLett.52.997' on page 48 undefined on input line
 130.


LaTeX Warning: Citation 'PhysRevA.38.1149' on page 48 undefined on input line 1
30.


LaTeX Warning: Citation 'maitra2003current' on page 48 undefined on input line 
130.


Overfull \hbox (2.78044pt too wide) in paragraph at lines 130--131
\OT1/cmr/m/n/12 dependent vec-tor po-ten-tial is present Ghosh and Dhara [[]

Overfull \hbox (38.10458pt too wide) in paragraph at lines 130--131
\OT1/cmr/m/n/12 and the vec-tor po-ten-tial. More re-cently Maitra and co-worke
rs [[]
[48]

LaTeX Warning: Reference `eq:dpftks' on page 49 undefined on input line 139.

[49]

LaTeX Warning: Reference `eq:tdksh' on page 50 undefined on input line 175.


LaTeX Warning: Citation 'maitra2003current' on page 50 undefined on input line 
176.


LaTeX Warning: Reference `eq:ksfld' on page 50 undefined on input line 184.


LaTeX Warning: Reference `eq:totfld' on page 50 undefined on input line 184.


LaTeX Warning: Citation 'PhysRevB.85.045134' on page 50 undefined on input line
 184.


LaTeX Warning: Reference `appA' on page 50 undefined on input line 184.


LaTeX Warning: Citation 'libxc' on page 50 undefined on input line 186.


LaTeX Warning: Citation 'aulbur1996polarization' on page 50 undefined on input 
line 186.


LaTeX Warning: Citation 'maitra2003current' on page 50 undefined on input line 
186.


LaTeX Warning: Citation 'PhysRevLett.115.137402' on page 50 undefined on input 
line 186.


LaTeX Warning: Citation 'maitra2003current' on page 50 undefined on input line 
187.


LaTeX Warning: Citation 'PhysRevLett.115.137402' on page 50 undefined on input 
line 187.


LaTeX Warning: Citation 'maitra2003current' on page 50 undefined on input line 
191.


Overfull \hbox (67.15913pt too wide) in paragraph at lines 186--192
\OT1/cmr/m/n/12 po-lar-i-sa-tion $\OT1/cmr/bx/n/12 p$ \OT1/cmr/m/n/12 (see for 
ex-am-ple Refs. [[] ], [[]
[50]

LaTeX Warning: Reference `Excmac' on page 51 undefined on input line 205.


LaTeX Warning: Citation 'maitra2003current' on page 51 undefined on input line 
205.

[51]

LaTeX Warning: Citation 'PhysRevLett.115.137402' on page 52 undefined on input 
line 212.


LaTeX Warning: Citation 'PhysRevLett.115.137402' on page 52 undefined on input 
line 212.


LaTeX Warning: Citation 'LRC' on page 52 undefined on input line 227.


LaTeX Warning: Citation 'PhysRevB.72.125203' on page 52 undefined on input line
 227.


LaTeX Warning: Citation 'PhysRevLett.114.146402' on page 52 undefined on input 
line 227.


LaTeX Warning: Citation 'PhysRevLett.107.186401' on page 52 undefined on input 
line 227.


LaTeX Warning: Reference `Excmac' on page 52 undefined on input line 229.


LaTeX Warning: Citation 'jgm' on page 52 undefined on input line 229.


LaTeX Warning: Citation 'jgm' on page 52 undefined on input line 231.

[52]

LaTeX Warning: Citation 'PhysRevB.57.14569' on page 53 undefined on input line 
236.


LaTeX Warning: Reference `eq:alpha' on page 53 undefined on input line 246.


LaTeX Warning: Citation 'jgm' on page 53 undefined on input line 247.


LaTeX Warning: Reference `eq:krnl' on page 53 undefined on input line 250.


LaTeX Warning: Reference `Excmac' on page 53 undefined on input line 250.


LaTeX Warning: Reference `Excmic' on page 53 undefined on input line 250.


LaTeX Warning: Reference `eq:pot_from_exc' on page 53 undefined on input line 2
50.


LaTeX Warning: Reference `Excmic' on page 53 undefined on input line 259.


LaTeX Warning: Reference `eq:krnl' on page 53 undefined on input line 259.


LaTeX Warning: Reference `eq:Excapp' on page 53 undefined on input line 259.

[53]

LaTeX Warning: Citation 'abinit' on page 54 undefined on input line 265.


LaTeX Warning: Citation 'gruningtddf1' on page 54 undefined on input line 265.


LaTeX Warning: Citation 'gonze' on page 54 undefined on input line 314.


LaTeX Warning: Reference `eq:proj' on page 54 undefined on input line 324.


LaTeX Warning: Citation 'souza_prb' on page 54 undefined on input line 324.


LaTeX Warning: Citation 'souza_prb' on page 54 undefined on input line 325.


LaTeX Warning: Citation 'nloptics2013' on page 54 undefined on input line 325.


LaTeX Warning: Citation 'PhysRevB.89.081102' on page 54 undefined on input line
 325.


LaTeX Warning: Reference `eq:wkhat2' on page 54 undefined on input line 325.


Overfull \hbox (43.23853pt too wide) in paragraph at lines 323--342
\OT1/cmr/m/n/12 In the def-i-ni-tion for the pro-jec-tor [Eq.[]] $\OMS/cmsy/m/n
/12 j[]i$ \OT1/cmr/m/n/12 are gauge-covariant,[[]

LaTeX Warning: Reference `eq:tdksh' on page 54 undefined on input line 347.

[54] <Abs.pdf, id=750, 483.51263pt x 432.28438pt> <use Abs.pdf>

LaTeX Warning: Citation 'gruningtddf1' on page 55 undefined on input line 375.


LaTeX Warning: Citation 'gruningtddf1' on page 55 undefined on input line 375.


LaTeX Warning: Citation 'PhysRevB.36.4821' on page 55 undefined on input line 3
81.


LaTeX Warning: Citation 'PhysRevB.35.9174' on page 55 undefined on input line 3
81.


LaTeX Warning: Citation 'Adachi' on page 55 undefined on input line 381.


LaTeX Warning: Citation 'GARRIGA' on page 55 undefined on input line 381.


LaTeX Warning: Reference `fg:epsblk' on page 55 undefined on input line 381.


Overfull \hbox (75.08086pt too wide) in paragraph at lines 381--383
\OT1/cmr/m/n/12 The ex-per-i-men-tal op-ti-cal spec-tra on Si [[] ], GaAs [[]

LaTeX Warning: Reference `fg:epsblk' on page 55 undefined on input line 384.


LaTeX Warning: Citation 'botti2007time' on page 55 undefined on input line 384.



LaTeX Warning: Citation 'Onida' on page 55 undefined on input line 384.


LaTeX Warning: Citation 'gruningtddf1' on page 55 undefined on input line 385.


LaTeX Warning: Citation 'PhysRevLett.43.387' on page 55 undefined on input line
 385.


LaTeX Warning: Citation 'PhysRevB.21.4656' on page 55 undefined on input line 3
85.


LaTeX Warning: Citation 'botti2007time' on page 55 undefined on input line 385.



LaTeX Warning: Citation 'Onida' on page 55 undefined on input line 385.

[55] <Abs2.pdf, id=758, 483.51263pt x 432.28438pt> <use Abs2.pdf>

LaTeX Warning: Citation 'gruningtddf1' on page 56 undefined on input line 392.


LaTeX Warning: Citation 'gruningtddf1' on page 56 undefined on input line 392.


LaTeX Warning: Reference `fg:epsblk1' on page 56 undefined on input line 396.


LaTeX Warning: Reference `sc:ksef' on page 56 undefined on input line 396.


LaTeX Warning: Citation 'gruningtddf1' on page 56 undefined on input line 397.


LaTeX Warning: Reference `fg:effG' on page 56 undefined on input line 397.

[56 <./Abs.pdf>]

LaTeX Warning: Citation 'boyd' on page 57 undefined on input line 403.


LaTeX Warning: Reference `fg:shg' on page 57 undefined on input line 403.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 57 undefined on input line
 407.

<SHG.pdf, id=804, 488.82153pt x 664.9938pt> <use SHG.pdf>

LaTeX Warning: Citation 'PhysRevB.82.235201' on page 57 undefined on input line
 410.


LaTeX Warning: Citation 'bergfeld2003second' on page 57 undefined on input line
 410.


LaTeX Warning: Citation 'Shoji:97' on page 57 undefined on input line 410.


LaTeX Warning: Citation 'Jang:13' on page 57 undefined on input line 410.


LaTeX Warning: Citation 'gruningtddf1' on page 57 undefined on input line 410.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 57 undefined on input line
 410.


LaTeX Warning: Citation 'bergfeld2003second' on page 57 undefined on input line
 410.


LaTeX Warning: Citation 'Shoji:97' on page 57 undefined on input line 410.


LaTeX Warning: Citation 'Jang:13' on page 57 undefined on input line 410.


LaTeX Warning: Citation 'gruningtddf1' on page 57 undefined on input line 410.


Overfull \hbox (6.26018pt too wide) in paragraph at lines 403--411
\OT1/cmr/m/n/12 In zincblende struc-tures the only in-de-pen-dent non-zero SHG 
com-po-nent [[]

Underfull \vbox (badness 10000) has occurred while \output is active [57 <./Abs
2.pdf>] [58]
Underfull \vbox (badness 10000) has occurred while \output is active [59]

LaTeX Warning: Citation 'PhysRevB.82.235201' on page 60 undefined on input line
 413.


LaTeX Warning: Citation 'nloptics2013' on page 60 undefined on input line 413.


LaTeX Warning: Reference `eq:wkhat2' on page 60 undefined on input line 413.


LaTeX Warning: Reference `fg:shg' on page 60 undefined on input line 413.


LaTeX Warning: Citation 'PhysRevB.82.235201' on page 60 undefined on input line
 414.


Overfull \hbox (39.75519pt too wide) in paragraph at lines 413--415
\OT1/cmr/m/n/12 ob-tained from a re-sponse ap-proach by Luppi and co-workers [[
]

Overfull \hbox (45.17819pt too wide) in paragraph at lines 413--415
\OT1/cmr/m/n/12 ] and we found a good agree-ment, slightly bet-ter than our pre
-vi-ous work[[]

Overfull \hbox (14.96538pt too wide) in paragraph at lines 413--415
\OT1/cmr/m/n/12 ] thanks to the higher or-der ap-prox-i-ma-tion for the co-vari
-ant deriva-tive [Eq. []].

Underfull \vbox (badness 10000) has occurred while \output is active [60 <./SHG
.pdf>]

LaTeX Warning: Reference `fg:siX3ab' on page 61 undefined on input line 420.


LaTeX Warning: Citation 'Moss:89' on page 61 undefined on input line 420.

[61] <X3.pdf, id=930, 481.6855pt x 435.44527pt> <use X3.pdf>

LaTeX Warning: Citation 'gruningtddf1' on page 62 undefined on input line 427.


LaTeX Warning: Citation 'gruningtddf1' on page 62 undefined on input line 427.


LaTeX Warning: Citation 'Moss:89' on page 62 undefined on input line 429.


LaTeX Warning: Reference `fg:siX3an' on page 62 undefined on input line 429.


LaTeX Warning: Reference `fg:siX3ab' on page 62 undefined on input line 429.


LaTeX Warning: Citation 'Moss1990' on page 62 undefined on input line 429.

[62 <./X3.pdf>] <anysX3.pdf, id=984, 578.16pt x 433.62pt> <use anysX3.pdf>

LaTeX Warning: Citation 'Moss:89' on page 63 undefined on input line 434.


LaTeX Warning: Citation 'gruningtddf1' on page 63 undefined on input line 434.


LaTeX Warning: Citation 'Moss:89' on page 63 undefined on input line 434.


LaTeX Warning: Citation 'gruningtddf1' on page 63 undefined on input line 434.


LaTeX Warning: Reference `fg:epsanl' on page 63 undefined on input line 440.


LaTeX Warning: Reference `fg:epsanl' on page 63 undefined on input line 441.

<Analysis.pdf, id=985, 578.16pt x 433.62pt> <use Analysis.pdf>

LaTeX Warning: Citation 'gruningtddf1' on page 63 undefined on input line 446.


LaTeX Warning: Citation 'gruningtddf1' on page 63 undefined on input line 446.

[63]

LaTeX Warning: Citation 'souza_prb' on page 64 undefined on input line 451.


LaTeX Warning: Citation 'Gonze1995' on page 64 undefined on input line 452.


LaTeX Warning: Citation 'Resta1996' on page 64 undefined on input line 452.


LaTeX Warning: Citation 'Vanderbilt1997' on page 64 undefined on input line 452
.


LaTeX Warning: Citation 'Martin1997' on page 64 undefined on input line 452.


LaTeX Warning: Citation 'LRC' on page 64 undefined on input line 453.


LaTeX Warning: Citation 'jgm' on page 64 undefined on input line 453.


LaTeX Warning: Citation 'LRC' on page 64 undefined on input line 454.


LaTeX Warning: Citation 'gruningtddf2' on page 64 undefined on input line 455.


Overfull \hbox (9.44217pt too wide) in paragraph at lines 451--456
\OT1/cmr/m/n/12 DPFT in-tro-duced in the nineties [[]; []; [];
[64]

LaTeX Warning: Citation 'PhysRevB.62.7998' on page 65 undefined on input line 4
57.


LaTeX Warning: Citation 'PhysRevB.85.045134' on page 65 undefined on input line
 457.


LaTeX Warning: Citation 'goncharov2013nonlinear' on page 65 undefined on input 
line 457.


LaTeX Warning: Citation 'PhysRevB.52.14636' on page 65 undefined on input line 
457.


LaTeX Warning: Citation 'tokman' on page 65 undefined on input line 457.

<Geff.pdf, id=997, 578.16pt x 433.62pt> <use Geff.pdf>

LaTeX Warning: Citation 'gruningtddf1' on page 65 undefined on input line 461.


LaTeX Warning: Citation 'gruningtddf1' on page 65 undefined on input line 461.


Overfull \hbox (34.2558pt too wide) in paragraph at lines 457--465
\OT1/cmr/m/n/12 have shown promis-ing results,[[]; []

LaTeX Warning: Citation 'PhysRevB.68.205112' on page 65 undefined on input line
 466.

) [65] [66] [67 <./anysX3.pdf>] [68 <./Analysis.pdf> <./Geff.pdf

pdfTeX warning: pdflatex (file ./Geff.pdf): PDF inclusion: multiple pdfs with p
age group included in a single page
>] (./conclusions.tex
Chapter 4.

Underfull \hbox (badness 10000) in paragraph at lines 2--3

[69]
Overfull \hbox (22.69862pt too wide) in paragraph at lines 11--13
\OT1/cmr/m/n/12 put-ing Ser-vice (http://www.archer.ac.uk) through EP-SRC grant
 EP/K0139459/1
) [70] (./appendix.tex
Appendix A.

LaTeX Warning: Reference `linear_response' on page 71 undefined on input line 9
.

[71]

LaTeX Warning: Citation 'schwegler:9708' on page 72 undefined on input line 42.



LaTeX Warning: Citation 'faber2014excited' on page 72 undefined on input line 4
2.

[72]
Appendix B.

Overfull \hbox (2.85518pt too wide) in paragraph at lines 49--53
\OT1/cmr/m/n/12 scopic di-elec-tric func-tion or of re-lated re-sponse func-tio
ns of di-electrics. Within
[73] [74] <pol_eps_and_eels.pdf, id=1184, 902.27875pt x 498.43402pt>
<use pol_eps_and_eels.pdf>

LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: Citation 'PhysRevB.85.045134' on page 75 undefined on input line
 175.


LaTeX Warning: Reference `induced' on page 75 undefined on input line 176.


LaTeX Warning: Reference `eq:tsusc1' on page 75 undefined on input line 176.


LaTeX Warning: Reference `eq:susc1' on page 75 undefined on input line 176.

[75] [76 <./pol_eps_and_eels.pdf>]
Appendix C.
(/usr/share/texlive/texmf-dist/tex/latex/base/omscmr.fd) [77]) [78]

LaTeX Warning: Empty bibliography on input line 276.

(./hdr.aux (./introduction.aux) (./realtime.aux) (./tddft.aux)
(./conclusions.aux) (./appendix.aux))

Package rerunfilecheck Warning: File `hdr.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.


LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package biblatex Warning: Please (re)run Biber on the file:
(biblatex)                hdr
(biblatex)                and rerun LaTeX afterwards.

 )
(see the transcript file for additional information)pdfTeX warning (dest): name
{equation.2.4.31} has been referenced but does not exist, replaced by a fixed o
ne

pdfTeX warning (dest): name{equation.2.4.23} has been referenced but does not e
xist, replaced by a fixed one

pdfTeX warning (dest): name{equation.2.4.22} has been referenced but does not e
xist, replaced by a fixed one

pdfTeX warning (dest): name{section.2.8} has been referenced but does not exist
, replaced by a fixed one

pdfTeX warning (dest): name{section.2.7} has been referenced but does not exist
, replaced by a fixed one

pdfTeX warning (dest): name{section.2.6} has been referenced but does not exist
, replaced by a fixed one

</usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmbsy10.pfb></usr
/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cmextra/cmbsy8.pfb></usr/
share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/
texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/share/texliv
e/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx6.pfb></usr/share/texlive/texmf
-dist/fonts/type1/public/amsfonts/cm/cmbx8.pfb></usr/share/texlive/texmf-dist/f
onts/type1/public/amsfonts/cm/cmcsc10.pfb></usr/share/texlive/texmf-dist/fonts/
type1/public/amsfonts/cm/cmex10.pfb></usr/share/texlive/texmf-dist/fonts/type1/
public/amsfonts/cm/cmmi10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public
/amsfonts/cm/cmmi12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmmi6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/
cmmi7.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi8.p
fb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmib10.pfb></
usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/sha
re/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr12.pfb></usr/share/texl
ive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr5.pfb></usr/share/texlive/texm
f-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb></usr/share/texlive/texmf-dist/f
onts/type1/public/amsfonts/cm/cmr7.pfb></usr/share/texlive/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr8.pfb></usr/share/texlive/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm
/cmsy7.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy8.
pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmti10.pfb></
usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmti12.pfb></usr/sh
are/texlive/texmf-dist/fonts/type1/public/amsfonts/symbols/msbm10.pfb>
Output written on hdr.pdf (78 pages, 2453880 bytes).
Transcript written on hdr.log.


==> REALTIME/realtime.tex <==
\chapter{Correlation from non-equilibrium Green's functions} 
\label{chaptercorr}
\section{A simple introduction to non-equilibrium Green's functions}
In this section we present a simple introduction to the non-equilibrium Green's functions, following the lines of Ref.~\cite{kremp}. \\

